Safe Grasping with a Force Controlled Soft Robotic Hand

Safe yet stable grasping requires a robotic hand to apply sufficient force on the object to immobilize it while keeping it from getting damaged. Soft robotic hands have been proposed for safe grasping due to their passive compliance, but even such a hand can crush objects if the applied force is too high. Thus for safe grasping, regulating the grasping force is of uttermost importance even with soft hands. In this work, we present a force controlled soft hand and use it to achieve safe grasping. To this end, resistive force and bend sensors are integrated in a soft hand, and a data-driven calibration method is proposed to estimate contact interaction forces. Given the force readings, the pneumatic pressures are regulated using a proportional-integral controller to achieve desired force. The controller is experimentally evaluated and benchmarked by grasping easily deformable objects such as plastic and paper cups without neither dropping nor deforming them. Together, the results demonstrate that our force controlled soft hand can grasp deformable objects in a safe yet stable manner.

==> IEEE SMC - Soft Hand Paper/acronyms.tex <==
\newacro{bn}[BN]{Batch Normalization}
\newacro{relu}[ReLU]{Rectified Linear Unit}
\newacro{adam}[Adam]{Adaptive Moment Estimation}
\newacro{ai}[AI]{Artificial Intelligence}
\newacro{dl}[DL]{Deep Learning}
\newacro{dnn}[DNN]{Deep Neural Network}
\newacro{cnn}[CNN]{Convolutional Neural Network}
\newacro{bnn}[BNN]{Bayesian Neural Network}
\newacro{mc}[MC]{Monte-Carlo}
\newacro{dof}[DOF]{Degrees-Of-Freedom}
\newacro{ods}[USN]{Uncertain Shape Network}
\newacro{od}[SN]{Shape Network}
\newacro{gp}[GP]{Gaussian Processes}
\newacro{mcmc}[MCMC]{Markov Chain Mote Carlo}
\newacro{psdf}[p-SDF]{probabilistic Signed Distance Function}
\newacro{gpis}[GPISs]{Gaussian Process Implicit Surfaces}
\newacro{va}[V]{Varley}
\newacro{spa}[SPA]{Soft Pneumatic Actuator}
\newacro{fsr}[FSR]{Force Sensitive Resistive}
\newacro{pwm}[PWM]{Pulse Width Modulation}
\newacro{rms}[RMS]{Root Mean Square}

\newacro{pi}[PI]{Proportional-Integral}
\newacro{pid}[PID]{Proportional-Integral-Derivative}
\newacro{bic}[BIC]{Bayesian Information Criterion}
\newacro{fem}[FEM]{Finite Element Method}
\newacro{ols}[OLS]{Ordinary Least Squares}

==> IEEE SMC - Soft Hand Paper/macro.tex <==
\newcommand{\miss}[1]{\todo[inline,color=yellow!30]{\textit{#1}}}
\newcommand{\ville}[1]{\todo[inline,color=green!30]{Ville: #1}}
\newcommand{\jens}[1]{\todo[inline,color=blue!30]{Jens: #1}}
\newcommand{\tran}[1]{\todo[inline,color=red!30]{Tran: #1}}

\newcommand{\figref}[1]{\hyperref[#1]{Fig.~\ref*{#1}}}
\newcommand{\tabref}[1]{\hyperref[#1]{Table~\ref*{#1}}}
\newcommand{\secref}[1]{\hyperref[#1]{Section~\ref*{#1}}}
\newcommand{\algoref}[1]{\hyperref[#1]{Algorithm~\ref*{#1}}}
\newcommand{\figsref}[2]{Figures~\ref{#1}-\ref{#2}}
\newcommand{\subfigref}[1]{(\subref{#1})}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\newcommand{\tbs}[1]{\renewcommand{\tabcolsep}{#1pt}}
\newlength\myindent
\setlength\myindent{2em}
\newcommand\bindent{%
	\begingroup
	\setlength{\itemindent}{\myindent}
	\addtolength{\algorithmicindent}{\myindent}
}
\newcommand\eindent{\endgroup}

\newcommand{\matr}[1]{\mathbf{#1}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\de}[1]{\operatorname{d}\!#1}

\def\bestcolor{(best viewed in color)}
\def\panda{\textit{Franka Emika Panda}}
\def\barrett{\textit{Barrett hand}}
\def\sota{state-of-the-art}
\def\spashort{\ac{spa} SPA}
\def\shapehypo{shape hypothesis}
\def\meanshape{mean shape}
\def\ie{\textit{i.e.,}}
\def\eg{\textit{e.g.,}}
\def\etal{\textit{et al.}}
\def\graspit{GraspIt!}
\def\pc{point-cloud}
\def\rbo{RBO Hand 2}
\def\dlr{DRL Soft Hand}
\def\ourhand{our soft hand}

\def\epst{\multicolumn{1}{c}{$\epsilon$}}
\def\vt{\multicolumn{1}{c}{$v$}}
\def\nat{\multicolumn{1}{c}{--}}

%%%%%%%% CUSTOM COLOR definitions
\definecolor{significant}{RGB}{217,217,217}
\definecolor{verysignificant}{RGB}{255,255,255}

==> IEEE SMC - Soft Hand Paper/sections/conclusion.tex <==
\section{CONCLUSIONS}
\label{ch:Conclusion}

We presented a force controlled soft robotic hand and used it for safe grasping. The key component was to integrate both resistive bend and force sensors onto the hand's fingers and apply a data-driven method to estimate the actual contact force between the fingers and the objects. The estimated contact force was then fed into a \ac{pi} force controller to keep a constant grasping force. We experimentally validated our force controller by comparing it to no force controller on a grasping experiment where the objective was to grasp deformable objects in a stable manner without damaging them. The results show that the force controlled soft hand could grasp the tested objects without neither dropping them nor causing significant deformation.

All in all, the work presented here demonstrates that applying a data-driven calibration method can make otherwise unreliable force sensor readings reliable enough to be used in a force feedback controller. This, in turn, poses new interesting research questions. For instance, is it possible to learn an accurate dynamics model from the force and bend data? If so, can such a model be used to do dexterous manipulation by a soft robotic hand with, \eg{} model predictive control or model-based reinforcement learning? Dexterous manipulation, together with the safety inherited from the softness properties of soft hands offer great potential for robots to interact with human in complex environments. 
% These questions pave the way for future research avenues.  


% This work, together with the proposed future works, will contribute towards expanding the application of soft robotic hands, including more sophisticated manipulation tasks. This, together with the safety inherited from the softness properties of the hand might leads to more service robots in human environments.

%However, the implemented system in this work also had its limitations. A key feature of the proposed approach is that it relies only on the feedback from the sensors that are directly integrated into the hand. Although the approach provides a general solution for enabling force control of any soft hands integrated with the same type of sensor, the system may not react fast and good enough to handle external disturbances such as pressure leaks. Another limitation of the system was the object deformation tracking as at the moment the deformation of objects was observed manually by the human. With all of this in mind, future extensions to improve the system developed in this work should concentrate on:
%\begin{enumerate*}[label=(\roman*)]
%    \item considering the feedback from the internal pressure sensor as another input for estimating the actual contact force. This helps to provide a more robust system that can handle external disturbances in terms of pressure leaks.
%    \item learning the minimum grasping force for different deformable objects by adding the object deformation detection by visual information from a high rate camera.
%\end{enumerate*}
%\tran{Jens, do you think the latter content is needed?}
%Further possibility for a soft robotic hand with embedded sensors is to estimate the properties of the grasped objects. As an additional experiment conducted in [my thesis?] proved the possibility of estimating the stiffness of an object, this can be further studied and expanded to other properties of the grasped objects such as size, shape, position, and orientation. Another interest research question is that is it possible for a soft robotic hand with embedded sensors to achieve complex manipulation tasks such as in-hand manipulation.

%The objectives of this thesis were to integrate appropriate sensors into a soft robotic hand and to develop a control strategy using only the sensory feedback for investigating the interaction between the soft hand and objects. Achieving these goals is a step towards showing that soft hands are able to not only grasp in the same manner as humans but also perform useful actions with grasped objects. 

%From the background theory, we observed that the majority of the works on soft robotic hands focus on the hand design rather than the control aspect. Soft hands were usually claimed to successfully grasp a wide range of objects. However, the target objects were typically rigid. This raised a question of whether we can manipulate deformable objects with soft hands. To accomplish this task, the interaction between the hand and objects (or contact force) is vital as deformable objects can be easily crushed even with soft hands when high contact force is used. Therefore, this work attempted to tackle this problem by integrating sensing capability into the soft hand to study the interaction between the soft hand and objects. In this work, we focus on selecting suitable sensors, then characterizing them to extract the desired information, in this case, contact force, and studying how to control the contact force to achieve complex manipulation tasks.

%The research methodology part started by presenting the characterization process of the chosen sensors: resistive flex bend and force sensor. While the bend sensor provided reliable data, the force sensor introduced a problem of producing internal force measurement when it is bent. To combat this issue, we proposed the method discussed in Chapter?? to estimate the actual contact force from the sensory feedback. The contact force estimating and the design of the proposed control strategy represent the core of this work. The sensing of contact force allows the detection of contact between the soft hand with objects or the environment. The control strategy used the switching control mechanism to choose the appropriate controller for each phase of the grasping, improving the quality of the grasp. Specifically, the force controller was activated only when the contact between the hand and objects was detected. 

%The performance of the proposed approach was tested in the experiments using the developed soft hand and controller board. The results were satisfactory. The proposed approach was able to control the contact force in real-time, using only sensory feedback from selected sensors. Nevertheless, the implemented system in this work also had its limitations. For the sensors, while the bend sensor provided valuable readings, the force sensor introduced a problem when it is bent. In addition, more complex manipulation tasks such as in-hand manipulation required the force measurements at different sections of the finger while the selected force sensor gave only one measurement along the body of the finger. Another limitation of the system was the object deformation tracking as at the moment the deformation of objects was observed manually by the human. With all of this in mind, future extensions to improve the system built in this thesis should concentrate on:
%\begin{itemize}
%    \item considering the feedback from the internal pressure sensor as another input for estimating the actual contact force. This helps to provide a more robust system that can handle external disturbances in terms of pressure leaks.
%    \item adding the object deformation detection by visual information from a high rate camera.
%    \item learning the minimum grasping force for deformable objects. In this work, the minimal grasping force for each object was found manually by experimenting with different values. With the development of the suggested object deformation detection, the minimal grasping force of different objects can be learned.
%\end{itemize}
%Other possibilities for a soft robotic hand with embedded sensors, which may be different from the one used in this thesis, are to:
%\begin{itemize}
%    \item estimate the properties of the grasped objects. As the experiment conducted in Section?? proved the possibility of estimating the stiffness of an object, this can be further studied and expanded to other properties of the grasped objects such as size, shape, position, and orientation.
%    \item learn to achieve more complex manipulation tasks such as in-hand manipulation.
%\end{itemize}

%The research on achieving complex manipulation tasks such as in-hand manipulation using soft robotic hands are still limited. To achieve those tasks, sensory feedback and reinforcement learning are usually used. However, the lack of sensing capabilities and simulation model of soft robotic hands have constrained the research on this matter. This work proved that it is possible to study the interaction between the soft hand and objects using only simple and commercial sensors. Hopefully, with the development of simulation models of soft robotic hands and the sensors, the research on complex manipulation skills with soft robotic hands will progress further.  

%All in all, this thesis showed that the interaction between a soft robotic hand and objects or the environment in terms of contact force could be studied by integrating inexpensive commercial sensors to the hand. In addition, the thesis proved that the contact force could be successfully controlled in real-time to interact with objects. This work, together with the proposed future works, will contribute towards expanding the application of soft robotic hands, including more sophisticated manipulation tasks. This, together with the safety inherited from the softness properties of the hand might leads to more service robots in human environments.

==> IEEE SMC - Soft Hand Paper/sections/experiments.tex <==
\section{EXPERIMENTS AND RESULTS}
\label{sec:Experiments}

The main questions addressed experimentally were:
\begin{enumerate}
    \item What is the accuracy of the contact force estimation?
    \item What is the accuracy of the force controller?
    \item Does the force controlled soft hand enable safe grasping?
\end{enumerate}
In order to provide justified answers to these questions, we conducted three experiments. The first experiment examines the contact force estimation accuracy, the second one the proposed force controller accuracy while the third evaluates safe grasping in terms of grasping deformable objects without neither damaging nor dropping them.

\subsection{Experimental setup}
All the experiments were evaluated on a soft robotic hand embedded with the bend and force sensors mentioned in \secref{sec:sensing}. For the hand design, we used the same finger structure as \rbo{} \cite{deimel_rbo2_2016} but opted for a kinematic structure similar to the \dlr{} \cite{homberg_haptic_2015} as it allows power grasping. As a result, \ourhand{} consisted of three fingers, in which two fingers are on one side (we call them \textit{finger 1 and finger 2}), and one finger is on the opposite side (\textit{finger 3}). The final soft hand is shown in \figref{fig:resultfigure}. 

To pneumatically control the hand, we used the soft robotics toolkit controller platform\footnote{Fluidic Control Board, \url{https://softroboticstoolkit.com/book/control-board}}. The input pressure was regulated with \ac{pwm}, and the control rate was 60 Hz. However, at such a high control rate, the high-speed switching of \ac{pwm} caused the hand to vibrate, which consequently induced noise into the force readings. To decrease the noise, we implemented the pneumatic low pass filter proposed in \cite{memarian_lowpass_2015}.

%To suit the need of this work, the soft hand was designed based on the following requirements: 1) ease of fabrication and modification; 2) ability to attach different sensors; 3) capability of grasping a wide range of objects. Achieving these requirement requires a methodological approach to selecting the actuators and the kinematics of the hand. After evaluating the existing soft hands, we developed a soft hand that consisted of three individual fiber-reinforced actuators (RBO Hand 2 finger \cite{deimel_rbo2_2016}) embedded with bend and force sensors. The kinematics of the developed hand is inspired by the DRL hand in \cite{homberg_haptic_2015}, in which two fingers are on one side, and one finger is on the opposite side. \figref{fig:softhanddesign} shows the final soft hand used in the experiments.
%\begin{figure}[t]
%  \begin{center}
%    \includegraphics[width=0.48\textwidth]{figures/softhandesign.jpg}
%  \end{center}
%    \caption{A different view of the entire soft hand. Three fingers of the hand are numbered to ease the latter representation.}
%  \label{fig:softhanddesign}
%\end{figure}

%To control the soft hand embedded with sensors at different operating conditions, a controller platform was constructed. Since the soft fingers used in this work are pneumatic, controlling the pressure and the duration of the input pneumatic supply is needed. The controller platform was implemented based on the proposed design by the soft robotics toolkit\footnote{Fluidic Control Board, \url{https://softroboticstoolkit.com/book/control-board}}. The input pressure to the soft finger is regulated with PWM, which basically controls the opening and closing times of high-speed solenoid valves valves\footnote{\raggedright SMC-VQ110U-5M Solenoid valve,\url{https://www.smcpneumatics.com/VQ110U-5M.html}}, at a rate of 60 Hz by an Arduino board via serial messages sent from a ROS node. The embedded sensors are also interfaced with the Arduino board to provide the sensors' feedback at the rate of 100 Hz. Although PWM provides simple and fast means for varying the pressure supply to the soft finger, it has the disadvantage of producing non-smooth output pressure. The main reason is the mechanical switching of the high-speed valve when it is continuously opened and closed. Supplying the soft actuator with fluctuating pressure will cause vibrations in the body of the finger, which introduces noise to the embedded sensors. Noisy sensory feedback will cause problems in the accuracy of the predictive model and the controller that use such data. To mitigate this issue, we implemented the pneumatic low pass filter introduced in \cite{memarian_lowpass_2015} that is capable of reducing the magnitude of noise on pressure output as well as the feedback response from the embedded sensor. 
\subsection{Estimating contact force}
Our hypothesis is that the internal force is correlated to the curvature of the finger. To test this, we gathered force data at different bending angles for each finger. The data in \figref{fig:forceestimator} shows the force measurements for each finger at different bending angles. Although the data for each finger, such as bending angle range differ from each other due to the manual fabrication process, we can clearly see the correlation between the bending angle and the force. Next, we fitted a separate polynomial model \eqref{eq:polymodel} to the data for each finger. According to the \ac{bic} values presented in \figref{fig:forceestimator}, a fourth-degree polynomial fitted the data for each finger best, which is also indicated by the high $R^2$ values. 

Next, using the models to predict the internal force, we evaluated the accuracy of the estimated contact force in \eqref{contactforce_equation}. The steps of the experiment are illustrated in \figref{fig:estimation_acc}. The accuracy was measured by first actuating one finger to press against a scale until the reading on the scale reached a predefined target set to an arbitrary value such as 200 gram (approximately 2 N) in this case. Once the target was reached, the actual contact force was estimated by subtracting the predicted internal force from the force measurement obtained from the sensor. In addition, to evaluate the accuracy of the proposed method at different finger configurations, the distance $\mathbf{d}$ between the finger and the scale was increased after each experimental cycle.

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.45\textwidth]{figures/experiment.jpeg}
  \end{center}
    \caption{Steps of the experiment conducted to evaluate the accuracy of the estimated contact force using the proposed approach.}
  \label{fig:estimation_acc}
\end{figure}
% As proposed in \secref{sec:calib_contact_force_est}, we subtracted the predicted internal force obtained using the derived model (\secref{sec:calib_contact_force_est}) from the real force measurement from the sensor to estimate the actual contact force.
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.45\textwidth]{figures/ext200.png}
  \end{center}
    \caption{Contact force estimation result of the force sensor.}
  \label{fig:estimation_result}
\end{figure}

The estimated contact force against the reference contact force at different bending angles is plotted in \figref{fig:estimation_result}. Although the graph shows that the estimate contact force varies slightly around the actual contact force, the error only ranges from 0.01 to 0.15 N at most, which is within the tolerance for the objects we will later grasp. All in all, estimating the contact force by simply subtracting the internal force from the real measurement is sufficiently accurate. %The estimated contact force is later used to detect contact between the finger and objects. Due to the fluctuation of the estimation error, a certain threshold is set to safely detect contact between the finger and an external object. The value of the threshold is defined differently for different fingers according to their maximum value of the estimation error. 

\subsection{Force Control}
\label{sec:exp_force_controller}

%To control the soft hand to interact with objects at a specific contact force, a direct force controller was developed. The developed direct force controller is a Proportional - Integral (PI) controller attempting to maintain the desired force, mathematically expressed as,
%\begin{equation}
%    u(t) = K_p e(t) + K_i \int_{0}^{t} e(\tau) d\tau,
%\end{equation}
%where $K_p$, $K_i$ all non-negative, denote the coefficients for the proportional and integral terms respectively, u(t) is the control variable, $e = F_{target}-F_{current}$ denotes the force error, which is the difference between the target value and measured value, t is the time or instantaneous time (the present),
%$\tau$ is the variable of integration (takes on values from time 0 to the present t). For this force controller, the proportional and integral gains were set to $K_p$ = 10 and $K_i$ = 1.5, respectively, which were the values that were experimentally found to provide the best outcome. 
Before conducting the experiment, we experimentally fine-tuned the proportional $K_p$ and integral $K_i$ gains of the force controller to 10 and 1.5, respectively. To experimentally evaluate the accuracy and stability of the force controller, each finger had to reach and track a variable reference signal. First, a finger was actuated with 65 kPa pressure to make contact with a solid object. Then, the step reference signal was increased from 0 to 3 N, and after 60 seconds the reference signal was set to 2 N. The sensory feedback from the embedded sensors was continuously fed to the internal force predictive model to estimate the actual contact force. The difference between the target and current contact force was then fed to the \ac{pi} controller in \eqref{eq:force_controller_discrete} whose output was the corresponding amount to be added to (or subtracted from) the current duty cycle signal. The experiment was repeated 5 times.
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{figures/forcecontroller.png}
  \end{center}
    \caption{Contact force response of the finger to step reference signals.}
  \label{fig:forcecontroller}
\end{figure}
The contact force response of one finger is shown in \figref{fig:forcecontroller}. The force response of the finger closely followed the step reference signals with a \ac{rms} error of 0.1 N. Moreover, the settling time of the finger was roughly 400 ms.  
% In addition, a key feature of this controller is that it relies only on the feedback from the sensors (bend sensor and force sensor) that are directly integrated into the hand. Thus, the proposed method and approach can be used to control any soft hands integrated with the same type of sensor.

To enhance the robustness of the grasping system, the force controller should only be activated when contact is detected. One option to achieve this is to utilize a switching mechanism between position and force control. We experimentally tested such a switching mechanism by having a finger reach a target contact force of 2.5 N only after contact was made. Initially, the finger was slowly actuated from a duty cycle of 0\% until contact with a solid object was detected based on the estimated contact force. After contact was established, the force controller was activated to regulate the pressure to achieve the target contact force.
%\begin{algorithm}[t]
%\SetAlgoLined
% Calibrate the finger by recording sensory feedback upon open and close\;
% Set the target contact force\;
% \While{true}{
%  Close the hand slowly\;
%  Read feedback from bend and force sensors\;
%  Use polynomial regression to estimate the contact force\;
%  \If{Contact detected (estimated contact force $>$ threshold)}{
%   Calculate the error between the current contact force and target contact force\;
%   Feed the error to the PI controller\;
%   Calculate the output duty cycle based on the error\;
%   Use the output duty cycle to command the finger to close or open to achieve the target contact force\;
%   }
% }
% \tran{Do we need this?}
% \caption{Name}
% \label{alg:alg1}
%\end{algorithm}
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{figures/switchcontroller.png}
  \end{center}
    \caption{The top figure shows the change in duty cycle to achieve the desired contact force while the bottom figure shows the contact force response of the force controller. The yellow region illustrates the duration the force controller was activated, the red dashed line represents the target contact force of 2.5 N and the green arrow indicates the settling time.}
  \label{fig:controlstrategy}
\end{figure}

\begin{table*}[htb]
    \centering
    \ra{1.1}
    \caption{The grasping results for the deformable objects\label{tb:final_results}.}
        \begin{tabular}{@{}ccccccccccccc@{}}
        \toprule
        \multirow{2}{*}{\makecell{Target contact force \\ of the opposable finger (N)}}
        & \multicolumn{2}{c}{Empty plastic cup} & \multicolumn{2}{c}{Empty paper cup} & \\
        \cmidrule(lr){2-3}\cmidrule(lr){4-5}
        & Dropped percentage{} & Deformed percentage{} & Dropped percentage{} & Deformed percentage{} &  \\
        \midrule
        4& 0\% & 100\% & 0\% & 100\%\\
        3& 0\% & 100\% & 0\% & 80\%\\
        {2}& 0\% & 90\% & {\textbf{0\%}} & {\textbf{20\%}}\\
        1.5& 0\% & 40\% & 30\% & 10\%\\
        {1}& {\textbf{0\%}} & {\textbf{10\%}} &  80\% &  0\%\\
        0.5& 60\% & 0\% & 100\% & 0\%\\
    \bottomrule
    \end{tabular}
\end{table*}

The duty cycle output from the controller and the contact force response are shown in \figref{fig:controlstrategy}. From the top figure, one can conclude that to achieve the target contact force the controller used a duty cycle value in the range of 45\% - 55\%. The main reason for the fluctuating duty cycle originates from fluctuations in the estimated contact force response caused by residual oscillations in the sensory reading. From the bottom figure, it is observed that the contact force response settled to a value of approximately 2.5 N in roughly 800 milliseconds. The \ac{rms} error between the measured and the target contact force was 0.21 N. In conclusion, regardless of the small fluctuations in the measured contact force and the output duty cycle, the proposed control strategy was successful in controlling the finger to achieve a target contact force in reasonable settling time. Furthermore, the proposed control strategy did not overshoot at the time of contact. 

Together, all these results confirm that it is possible to control the interaction force between the soft hand and objects in a safe, accurate, and fast manner. Such features are of uttermost importance in safe grasping. 

\subsection{Safe Grasping} 
\label{sec:safe_grasping}
Based on the results from the previous experiments, our proposed force controller exhibits characteristics for safe grasping. In safe grasping, the goal is to grasp deformable objects that can easily deform, such as the plastic cup seen in \figref{fig:resultfigure}, in a stable manner. We experimentally evaluated if the proposed force controlled soft hand can do safe grasping by grasping three sensitive objects: an empty plastic cup, an empty paper cup, and an empty eggshell all shown in \figref{fig:finalexp}. Of these objects, the empty plastic and paper cup represents deformable objects while the empty eggshell represents a fragile object.

%The previous experiments were conducted to evaluate the characteristics of selected sensors and the behaviour of the proposed control strategy. The results of the experiments show that it is possible to control the contact force between a soft hand and objects using only the feedback from embedded sensors. However, the question of why do we need to integrate sensors to the soft hand to manipulate objects was not answered. To answer this question, a final experiment was conducted, and it examined if a soft hand can successfully grasp deformable objects such as empty plastic cup without crushing or dropping them using the selected sensors and the proposed control strategy. The key factor in this problem is the grasping force, too big a grasping force causes damage to the objects while too small a grasping force leads to a failed grasp attempt. Thus, to successfully grasp deformable planar objects, a suitable grasping force needs to be fed to the gripper. The final experiment was conducted to find the minimum grasping force for grasping deformable objects using the selected sensors and the proposed control strategy. In this experiment, three objects shown in Figure\ref{fig:finalexpobj}, \textit{i.e.}, an empty plastic cup, an empty paper cup and an empty eggshell, were used as target objects. 
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.4\textwidth]{figures/finalexp.jpg}
  \end{center}
    \caption{The target objects used in the safe grasping experiment.  \label{fig:finalexp}
}% from left to right: an empty plastic cup, an empty paper cup, and an empty eggshell.}
\end{figure}
% \vspace{-1mm}

%The empty plastic cup and the empty paper cup represent deformable objects and the empty eggshell a fragile object. 
For this experiment, the soft hand was fixed to a handle, as shown in \figref{fig:resultfigure}. As the soft hand had two fingers on one side and one on the opposite, to stabilize the objects the targets contact forces of the three fingers were set in such a way that the sum of the contact force of the two fingers was equal to that of the opposable finger. We tested six different force set-points for the opposable finger: $4$, $3$, $2$, $1.5$, $1$, and $0.5$ N. To evaluate a grasp, the hand first grasped the object until the target contact force was achieved and then we manually moved the handle upward 30 cm to lift the object and finally shook it randomly. During the process, a grasp was successful if the object neither deformed in the case of deformable objects nor broke in the case of fragile objects nor slipped away from the hand. We evaluated ten grasps for each target force amounting to 60 grasps in total. 

The grasping result on the deformable objects are presented in \tabref{tb:final_results}. As suspected, a higher contact force lowers the dropping rate but increases the deformation rate. The results show that even soft hands, which have been proposed for safe grasping due to their passive compliance, can completely deform objects if the force is too high. For instance, the plastic cup, which is less durable than the paper cup, can be deformed with as low a contact force as 1 N. The paper cup, on the other hand, can withstand up to 2 N of contact force. The minimum grasping force to successfully grasp deformable object can also be deduced from the results. 
% \jens{We should write a more about the results here.}

In addition, the experiment was also conducted on an empty eggshell to evaluate the proposed control strategy in the case of fragile objects. In this case, the eggshell never broke not even with maximum target contact forces. However, with a soft hand that can generate much larger grasping forces, crushing fragile objects is indeed feasible. All in all, the results emphasize the need for integrating sensors into soft hands to manipulate deformable and fragile objects. 


%Hence, simply grasping the objects with full force control, which is the case with no force-feedback, will completely crush the object as seen in Figure ??. However, to successfully grasp the object without crushing or dropping the objects, a contact force that provides the lowest dropped rate and the lowest deformed rate was desired. As the empty plastic cup is softer than the empty paper cup, the minimum force to successfully grasp the plastic cup should be smaller than that of the paper cup. This was proved by the result shown in the table, in which the minimum force in the case of the plastic cup (1 N) is half of the one for the paper cup (2 N). Furthermore, earlier result presented in \tabref{tb:final_results} shows that the deformable objects can be crushed even with soft hands when high force is used. Specifically, when we applied 2 N, 2 N, and 4 N of force, respectively to three fingers of the soft hand, both the empty plastic cup and the empty paper cup were crushed. This emphasizes the need for integrating sensors to soft hands to manipulate deformable objects.

%In addition, the experiment was also conducted on the eggshell to evaluate the proposed control strategy in the case of fragile objects. The result shows that the eggshell can not be damaged even with maximum contact forces in this case. Thus, a soft hand embedded with sensors seems to be redundant in the case of fragile objects. However, with a soft hand that can generate much larger contact forces, crushing fragile objects is indeed feasible. Furthermore, earlier results shown in \tabref{tb:final_results} show that the deformable objects can also be crushed even with soft hands when high force is used. Specifically, when we applied 2 N, 2 N, and 4 N of force, respectively to three fingers of the soft hand, both the empty plastic cup and the empty paper cup were crushed. This emphasizes the need for integrating sensors to soft hands to manipulate deformable planar objects. 

\subsection{Object properties estimation}
In addition to the previous experiments, we conducted one more extra experiment to show the potential of using the proposed soft hand to estimate object properties such as hardness. According to Yuan \cite{yuan16}, the most important factor to estimate the hardness of an object is the relationship between the geometry of the deformed object and the pressing force. When pressing on harder objects, they deform less compared to soft objects, thus retaining larger slopes on the contact surface \cite{yuan16}. In this work, the estimated contact force is seen as the pressing force, and the bending angle of the finger is considered as the deformation of the object. This experiment investigates whether the relationship between the two can be used to realize the hardness of an object.


For this experiment, the finger was fixed to a handle and actuated to make contact with two objects with different hardness \ie a solid spray can, and a woolly hat as shown in \figref{fig:softsolidobj}. The target objects were placed in such a way that they will be in contact with the finger at 40\% duty cycle. Both force and position sensory readings were then recorded for analysis.

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.3\textwidth]{figures/solfvssolidobj.jpg}
  \end{center}
    \caption{The top figure shows the two target objects in this experiment: a woolly hat and a spray can. Bottom figures show the experimental setup for both objects.}
  \label{fig:softsolidobj}
\end{figure}
\figref{fig:softvssolidbend} plots the relationship between the bending angle and the estimated contact force in both cases. The results show that in the case of the spray can the bend angle remains almost constant while the contact force continues to increase. This means that the finger has been stopped by something stiff. And since the finger is kept actuating, it keeps pressing stronger against that stiff object resulting in the increase of the contact force. However, in the case of the woolly hat, both the bending angle and the contact force increase simultaneously after the contact. This indicates that the target object is not stiff enough to constrain the bending of the finger after contact. Based on these results, it seems that the soft finger embedded with selected sensors can successfully distinguish between a solid object and a soft object using only the sensory feedback. 
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.5\textwidth]{figures/softvssolidbend.png}
  \end{center}
    \caption{The blue line represents the estimated contact force when the finger bends in free space. The orange and green line represent the estimated contact force when the finger makes contact with the spray can and the woolly hat, respectively.}
  \label{fig:softvssolidbend}
\end{figure}

==> IEEE SMC - Soft Hand Paper/sections/force_controller.tex <==
\section{FORCE CONTROLLER}
\label{sec:Force_controller}
To control the grasping force of the soft hand, we propose using a discrete \ac{pi} controller 
\begin{equation}
    u_n = K_p e_n + K_i T \sum_{k=1}^{n} e_k,
    \label{eq:force_controller_discrete}
\end{equation} 
where $K_p$ and $K_i$ are the proportional and integral terms respectively, $T$ is the sampling period, and $e_n$ is the force error between the target value and measured value at the n-th moment of sampling. The output $u_n$ is a \ac{pwm} signal. The reason why we chose to use a \ac{pi} controller instead of a \ac{pid} controller is that the derivative action is sensitive to noise. As the force measurement of the force sensor is usually noisy, the derivative action is neglected.

%\begin{equation}
%    u(t) = K_p e(t) + K_i \int_{0}^{t} e(\tau) d\tau,
%    \label{eq:force_controller_cont}
%\end{equation}
%where $K_p$ and $K_i$ are the proportional and integral terms respectively, $e$ is the force error between the target value and measured value, and $t$ is the instantaneous time. However, to conform to the digital force controller readings, we approximated \eqref{eq:force_controller_cont} as 

%For this force controller, the proportional and integral gains were set to $K_p$ = 10 and $K_i$ = 1.5, respectively, which were the values that were experimentally found to provide the best outcome. 


==> IEEE SMC - Soft Hand Paper/sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

A stable yet safe grasp requires a robotic hand to apply sufficient force on the target object to not harm it but still immobilize it. Recently, soft hands have been proposed for safe grasping due to their passive compliance. However, as shown in \figref{fig:resultfigure} even such hands can deform objects if the applied force is too high. There is, therefore, a need to control the grasping force also in soft hands. 

Research on soft hands has mainly focused on hand design \cite{schulz_anthrohand_2001,dollar_sdmhand_2010,filip_starfish_2011,deimel_rbo1_2013,deimel_rbo2_2016,galloway_underwater_gripper,zhou_40N_gripper,gecko_design,bryan19,nishimura19}. Only recently have works started to address the integration of sensing capabilities such as position \cite{elgeneidy_bendpredict_2018,chin_deform_19,gerboni_17,soter18} and force sensing \cite{homberg_robustgrsp_2019}. However, the authors found the existing solution for force sensing to be insufficient for contact detection, especially for small objects \cite{homberg_robustgrsp_2019}. In this work, we aim to show that force estimation is possible to allow both contact detection as well as control of contact forces for safe grasping.

To this end, we propose to integrate off-the-shelf resistive bend and force sensors in each finger of a hand to estimate the contact force and feed it into a force controller for each finger. In order to extract reliable force measurements, we propose a data-driven sensor characterization and calibration method for such sensors. Given the calibrated sensors, the real contact force is estimated by subtracting the residual force the sensor senses when bending in free space from the actual force reading. The residual force is also learned. The estimated force is then used in a \ac{pi} controller to control the set-point force for each finger. The complete force controller is experimentally validated and compared to no force controller on a physical grasping experiment where the objective is to grasp deformable and fragile objects in a stable manner without neither destroying nor deforming them.

The main contributions of this work are:
\begin{enumerate*}[label=(\roman*)]
	\item integration of resistive bend and force sensors in a soft hand (\secref{sec:sensing}), 
	\item calibration of the sensors to estimate contact force (\secref{sec:est_contact_force}),
	\item a force controller for the soft hand (\secref{sec:Force_controller}), and
	\item an empirical evaluation of the controller demonstrating that using a force controller deformable objects can be grasped in a stable yet safe manner (\secref{sec:Experiments}).
\end{enumerate*}
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{figures/resultfigure.jpg}
  \end{center}
    \caption{On the left is shown that grasping a fragile object with a high force will deform it completely while, as shown on the right, using force-feedback to control the grasping force this is no longer the case.}
  \label{fig:resultfigure}
\end{figure}
%For the past several decades, robots have shown great potential. For instance, robots are nowadays used extensively in complex environments such as homes, factory floors, or even hospitals. They come in different sizes and structures to perform various tasks from simple pick-and-place tasks to sophisticated surgeries on a human. The most common type of a robot is industrial manipulator. These robots are mainly seen at automated production lines on factory floors, where they must follow a predefined set of way-points to execute pick-and-place or assembly tasks on well-defined objects. The main reason robots work well in such a setting is that the environment and the objects are fully-known in advance and persistent for most of the time. However, the real world is not a predictable production line, where all objects to be manipulated and the end-effector target are known. For this reason, most of the research on robotic grasping is aimed at solving the problem of incomplete knowledge of objects and environment.
%What are soft robots? What are their potential applications?

%One popular approach that is currently intensively researched is to incorporate softness into robotic systems. The concept of creating robots from a highly compliant, \textit{i.e.}, low elastic modulus, material that can easily be stretched or distended \cite{vegas2013} is referred to as Soft Robotics \cite{trivedi08}. Due to the soft nature of the material, soft robots not only allow increased flexibility and adaptability for manipulating a wide range of objects but also enhance the safety when collaborating with humans \cite{rus15}.
%These unique characteristics enable soft robots to accomplish complex tasks in medical and manufacturing fields such as helping a patient in physical rehabilitation \cite{tse18}, creating prostheses for those missing limbs \cite{tse18}, or handling fresh fruits and vegetables \cite{britt2018} 
% Soft robotics in grasping. Good and bad!

%As compliance allows more intuitive grasping, softness is now built into robotic grippers for manipulating objects. Traditionally, to grasp with rigid hands, the knowledge of an object's properties and its location must be known in detail. Then grasp planning algorithms will generate the precise contact locations where to place each finger of the gripper to grasp the object. However, with soft robotic hands, the solution can be much simpler, more human-like, and thus perform better in handling uncertainty \cite{homberg2019}. Despite advantages of soft robots, one of their downsides is the absence of sensing capabilities, which leads to a limited range of applications. So far soft robotic hands are often used for simple manipulation tasks such as pick-and-place which do not need a complex controller and information of the hand's configuration \cite{khaled18}. Due to the compliance of the body, it is non-trivial to know the hand's configuration at a specific point of time, especially when being in contact with objects or interacting with the environment. This information is vital in grasping since it can be used to determine whether a grasp is stable and whether an object behaves as intended when grasped. Furthermore, the information can also be used together with machine learning to classify grasped objects \cite{homberg15} or even to perform dexterous manipulation \cite{gupta16}. Hence, to accomplish more sophisticated manipulation tasks, the sensing capabilities for soft robotic hands should be taken into account. 
%Thesis's goal and research question

%Despite extensive research in soft robotic grasping, the research on integrating sensing capabilities into soft robotic hands to achieve complex manipulation tasks is still limited. A majority of the works in soft robotics focus on the hand design \cite{sdmhand,bretthauer01,starfishgripper,rbo1,rbo2}, while some did integrate sensors into the hand but only limited to classifying objects \cite{homberg15} and position control \cite{khaled18} rather than to control the interaction between the object and the hand. The work presented in this thesis addresses the open problem on studying the interaction between the object and soft robotic hands using different sensors, \textit{i.e.}, bend and force sensors integrated into the hands. We address the following research questions:
%\begin{itemize}
%    \item How to effectively choose and integrate suitable sensors into a soft robotic hand?
%    \item How to calibrate and characterize the sensors to extract useful information, \textit{i.e.}, the actuator's curvature and contact force?
%    \item How to control the interaction between a soft hand and an object using the extracted information?
%\end{itemize}
%The need for using sensors to study the interaction between the soft hand and the object is demonstrated by performing an experiment that is challenging enough for both traditional rigid hands and soft hands without sensing capability. One suitable experiment for this demonstration is grasping deformable planar objects. The desired outcome is for robotic hands to successfully grasp the objects without dropping or crushing them. The most important factor in this problem is indeed the grasping force. If the grasping force is too small, the gripper will drop the object. On the other hand, too big a grasping force will cause damage to the object. Although a number of works on manipulating deformable planar objects have been conducted with traditional rigid hands, the problem remains because of limitations in hardware as well as control algorithms \cite{deformable_survey}. Another approach for grasping deformable planar objects is to use soft hands. However, the objects can also be easily crushed even with soft hand when high force is used. Therefore, sensing capability is needed for the soft hand to successfully achieve the goal.

==> IEEE SMC - Soft Hand Paper/sections/related_work.tex <==
\section{Related Work}
Most of the research in soft robotic hands has focused on the hand design itself where the main actuators have been the \ac{spa} \cite{shintake_softgripper_18}. \ac{spa}s are constructed of soft and deformable matter and are pneumatically actuated. Such actuators were used in the pioneering soft hand design by Ilievski \etal{} in 2011 \cite{filip_starfish_2011} where they presented a three-layer starfish inspired soft gripper using embedded pneumatic networks or PneuNets. The multilayer structures, where two active layers were separated by a passive layer, allowed the gripper to perform a wide range of motions, but due to its construction it could only withstand a small amount of pressure resulting in a weak grasping force. 

Recently, alternative soft hand designs that can attain higher grasping forces have been proposed, including the well known anthropomorphic \rbo{} \cite{deimel_rbo2_2016} and \dlr{} \cite{homberg_haptic_2015}. The \rbo{} consists of seven fiber-reinforced pneumatic continuum actuators acting as fingers and palm. Although the anthropomorphic design enabled dexterous grasping, one downside is the negative curvature of the thumb, meaning that the backside of the thumb is the primary contact surface rather than its front side, which makes it problematic to attach sensors to it. Compared to the \rbo{}, the kinematics of the \dlr{}, where two fingers are parallel and opposes the third, allow easy sensor integration and was, therefore, the source of inspiration for the hand proposed in this work. 

%To attain higher grasping force alternative soft hand designs such as the anthropomorphic \rbo{} \cite{deimel_rbo2_2016} consisting of seven fiber-reinforced pneumatic continuum actuators acting as fingers and palm. Although its anthropomorphic design enabled dexterous grasping, one downside of it is the negative curvature of the thumb, meaning that the backside of the thumb is the primary contact surface rather than its front side. Such a structure makes it problematic to attach sensors to the thumb. 
%A similar soft hand to the \rbo{} is the \dlr{} \cite{homberg_haptic_2015}. The kinematics of the \dlr{}, where two fingers are parallel and opposes the third, allows the hand to grasp a wide range of objects and resembles that of commonly used three-finger adaptive gripper such as the Barrett hand \cite{barrett_hand}. The kinematic structure of the \dlr{} also allows for easy sensor integration and was there fore the source of inspiration for the hand proposed in this work. 

Despite the wide range of research in soft hand designs, few works have studied how to incorporate sensing capabilities in such hands. One possible reason for the lack of research in sensorized soft hands is the few existing cheap off-the-shelf sensors that can be integrated into a \ac{spa}. However, recently Elgeneidy \etal{} \cite{elgeneidy_bendpredict_2018} proposed the following sensors for measuring and controlling position of \ac{spa}s: 
\begin{enumerate*}[label=(\roman*)]
	\item conductive elastomer sensors, 
	\item sensors made from liquid metal or
	\item resistive flex sensors.
\end{enumerate*}
%\subsection{Soft Hand Design}
% Two or three sentence about SPA, why it is chosen? And existing hand maybe?
%The soft hand consist of the actual actuation mechanics to bend and retract the hand and the design itself. In a recent overview by Rus \etal{} \cite{rus_control_2015} they list three different soft robot actuation methods: cable-driven, electroactive polymers, and fluidic (pneumatic or hydraulic). Today, one of the most common soft robotic actuator is a \ac{spa} \cite{shintake_softgripper_18} which is of a soft, deformable structure, and pneumatically actuated. Due to its characteristics such as intrinsic compliance, easy manufacturability and customization, \ac{spa}s makes it convenient and fast to integration sensing capabilities into itself.

%Many different soft hands build from \ac{spa}s exist in the literature. 
%For instance, the pioneering soft grippers by Ilievski \etal{} in 2011 \cite{filip_starfish_2011} is a starfish inspired soft gripper comprised of three layers using embedded pneumatic networks or PneuNets. The multilayer structures, where two active layers were separated by passive layers, allowed the gripper to perform a wide range of motions, but due to its construction it could only withstand small amount of pressure resulting in weak grasping force. 
% Many different soft hands build from \ac{spa}s exist in the literature. For instance, Ilievski \etal{} in 2011 \cite{filip_starfish_2011} developed a starfish inspired soft gripper, that can perform wide range of motion. 


%\subsection{Control of Soft Actuators}

%Despite extensive research in soft robotics, not much work has focused on accurate control of soft actuators. Most work on this subject utilized \ac{fem} to model the kinematics and dynamics of soft robots which are then used for control \cite{duriez_fem_2013},\cite{zhang_fem_16}. Although this approach enables accurate control of soft robots, \ac{fem} is computationally expensive and thus hard to achieve real-time control. However, one recent work \cite{largilliere_femreal_2015} proposed using asynchronous \ac{fem} which significately improved the real-time control performance. Another approach is to integrate flexible sensors directly onto soft hands to obtain feedback. Nevertheless, all previously mentioned methods only consider hand control in free space and not in contact which is the core focus of this paper.
% Lack in sensing integration -> 3 approaches -> Some work for each and drawbacks of the other 2 -> Choose resistive? Why? 
%\subsection{Sensorized Soft Hands}

Conductive elastomer sensors were used in \cite{petkovic_elastomer_2012} to control the displacement of the soft gripper with an adaptive neuro-fuzzy inference strategy. Unfortunately, the accuracy of such sensors quickly deteriorates as the distribution of carbon particles inside the elastomer material is disturbed by the actuator's repeated deformation. The more durable liquid metal sensors were integrated into a soft gripper in \cite{eGaIn_presence} to detect the presence of grasped objects, and in \cite{morrow_force_2016} to acquire pressure, force, and position data which was subsequently fed to a \ac{pid} controller to control the position of the finger and grasping force. However, to acquire the data, they used the eGain liquid metal sensor \cite{Park_eGaIn_2012} that was fabricated from scratch, which is a time-consuming and error-prone process. Additionally, the force sensor was placed at the tip of the actuator, restricting the force controller to only work with pincer grasps or on large objects. In this work, we target objects of diverse sizes, including small objects and as such the eGain sensor is not applicable.   

The third sensor type mentioned in  \cite{elgeneidy_bendpredict_2018}, the resistive bend flex sensors, are cheap, widely available, and easy to integrate in soft hands. For instance, resistive bend sensors have been used for haptic identification of grasped objects \cite{homberg_haptic_2015} and for predicting and controlling the position, \ie, bending angle of a pneumatic-driven actuator \cite{elgeneidy_bendpredict_2018}. The work in \cite{homberg_haptic_2015} was later improved in \cite{homberg_robustgrsp_2019} by adding a \ac{fsr} sensor to strengthen the grasp by detecting the contact between the hand and objects. They reported, however, that the force sensor provided unreliable data, resulting in extremely poor performance in contact detection, especially on small objects. This problem stems from placing the force sensor only at the tip of the finger, which will not make contact with small objects such as a tennis ball, resulting in no readings. In this work, we also use \ac{fsr}s due to their simplicity and availability but opt for the kinds that measure forces along a wider area as they enable measuring forces even on small objects.

==> IEEE SMC - Soft Hand Paper/sections/sensing_with_sensors.tex <==
\section{Resistive Based Sensing}
\label{sec:sensing}

%Typically, the internal pressure in the actuator is the only available feedback and it does not directly correlated to more useful information such as the position or the force applied to the actuator. 
%Robotic hands usually require position and force feedback to do complex manipulation tasks. 

To do complex manipulation tasks, robotic hands need position and force feedback \cite{manipulation_requirement}. To achieve this for soft hands, we propose integrating deformable resistive force and bend sensors onto the finger of the RBO Hand 2 proposed in \cite{deimel_rbo2_2016}. \figref{fig:sensorintegration} shows the sensors integrated into the fabricated actuator. The body of the fabricated actuator is divided into two parts: an extensible and an inextensible layer. 

% \footnote{\url{https://www.smooth-on.com/products/dragon-skin-10-medium/}}
To keep the bend sensor in place, it was encapsulated in the inextensible layer shown as the orange line in the figure. In contrast to the bend sensor, the force sensor illustrated by the green line in the figure needs to be in contact with the environment to get measurements; thus it was glued directly to the outer surface of the inextensible layer using freshly mixed Dragon Skin 10 silicone. Next, we describe the design and working principle of these sensors.
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{figures/sensorintegration.jpg}
  \end{center}
    \caption{A cross-sectional view of the actuator embedded with selected sensors.}
  \label{fig:sensorintegration}
\end{figure}
\subsection{Position sensing} 
\label{sec:pos_sensing}

To measure the internal state (position) of \ac{spa}s we used resistive flex sensors (bend sensors)\footnote{Flex Sensor 4.5": \url{https://www.sparkfun.com/products/8606}}. One side of the sensor consists of a layer of polymer ink which is embedded with conductive particles, as shown in \figref{fig:flexprin}. The particles provide the ink with a certain amount of resistance when the sensor is straight. When the sensor bends away from the ink, the conductive particles move further apart as shown in \figref{fig:flexprin} which, in turn, increases the resistance. Once the sensor return to the initial pose, the resistance also returns to the original value. Hence, the change in the resistance can be used to determine the curvature of the sensor.
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{figures/bendsensor.png}
  \end{center}
    \caption{The left figure shows the design of a resistive flex sensor and its behaviour in straight state. The right figure illustrates the behaviour of the sensor when it is bent in the right direction.}
  \label{fig:flexprin}
\end{figure} 

\subsection{Force sensing}
\label{sec:force_sensing}

To measure the grasping force applied by \ac{spa}s, we use \ac{fsr}s. \ac{fsr}s are designed to measure the presence and relative magnitude of localized physical pressure. The \ac{fsr} used to measure the force in \cite{homberg_robustgrsp_2019} was placed only at the tip of the finger but, given the fact that soft hands typically are developed to mimic human's grasping behaviour, \ie\ wrapping an entire finger around the surface of an object, placing the force sensor at such a location is not optimal for detecting contact between the hand and the object. Based on this, we opted for force sensors that can provide measurements along the body of the whole finger rather than only at the tip. To meet this requirement, we chose a strip \ac{fsr} with rectangle shape\footnote{Force Sensitive Resistor - Long
: \url{https://www.sparkfun.com/products/9674}}. The chosen sensor is a single large sensing taxel with the force sensitivity ranges from $0.01$ to $1000$ N. In addition, the force resolution of the sensor is better than $± 0.5 \%$ of full use force. 

An \ac{fsr} consists of a resistive polymer layer and a conductive film as illustrated in \figref{fig:fsrprin} and the working principle is similar to that of the bend sensor. Specifically, the spacer placed in between the two layers to avoid contact between them results in a very high resistance when no pressure is applied. When pressure is applied, the resistive polymer starts to make contact with the conductive film, which, in turn, reduces the resistance of the sensor. The stronger the applied force is on the sensor’s active area, the more the resistance between the two terminals drops. The actual applied force is mapped from the measured resistance using the resistance-force relationship graph provided in the datasheet of the sensor\footnote{https://cdn.sparkfun.com/datasheets/Sensors/Pressure/FSR408-Layout2.pdf}.

The design of the \ac{fsr} enables easy contact detection in stationary situations when the sensor is fixed to a surface. However, when the sensor is bent in free space the conductive and resistive polymer layer can come in contact with each other producing \textit{internal force readings} which leads to incorrect contact forces. In the next section, we propose a data-driven calibration method to correctly estimate the contact force by compensating for the internal force.

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{figures/forcesensor.png}
  \end{center}
    \caption{The left figure shows the design of a strip \ac{fsr} and its behavior when no pressure is applied. When pressure is applied on the sensor, the conductive particles move and make contact with the conductive film, resulting in more conduction paths (lowering resistance). }
\label{fig:fsrprin}
\end{figure}


==> IEEE SMC - Soft Hand Paper/sections/sensor_calibration.tex <==
%\section{SENSOR CALIBRATION}
%\label{sec:sensor_calibration}
% The detail information and the characterization process of each sensor are presented next.
%\subsection{Bend sensor}
%\label{sec:calib_bend_sensor}

%To quantify the bend sensor characteristics attached onto the soft finger  
%To calibrate the bend sensor attached to the soft finger, the finger was actuated by applying an input pressures from 0 kPa to approximately 60 kPa with three different actuating durations. Once the internal pressure in the finger reached 60 kPa, the finger was reset to its initial position by applying a 0 kPa input pressure. This procedure was repeated 35 times to evaluate the accuracy and the repeatability of the sensory readings. \figref{fig:bendsensor_char} plots the duty cycle input against the estimated bending angle of the bend sensor when inflating the finger for three different durations. 
%\begin{figure}[t]
%  \begin{center}
%    \includegraphics[width=0.48\textwidth]{figures/flexsensorchar.png}
%  \end{center}
%    \caption{The figure shows the bending angle against the duty cycle.}
%  \label{fig:bendsensor_char}
%\end{figure}

%The plotted cycle shows the bending angle of the sensor increases due to a higher internal pressure caused by an increased duty cycle. It is observable that the longer actuation duration, the more the readings fluctuate. In addition, longer actuation duration produces larger readings. The main reason is that during the actuation duration, the finger continues to bend rather than keeping the same position. The longer the actuation duration is, the more the finger bends which, in turn, increases the bending angle. Therefore, one can conclude that the reading of the bend sensor is slightly dependent on the actuation duration. Hence, to obtain stable readings of the bend sensor, suitable actuation duration needs to be carefully considered and selected.
\section{Data-Driven Contact Force Estimation}
\label{sec:est_contact_force}
%\subsection{Force sensor}
%\label{sec:calib_force_sensor}
%To calibrate the force sensor we applied objects with known masses of 108.20 gram on the body of the sensor. At first only one object was placed on the sensor but later several objects were placed along the body of the sensor to evaluate the sensing capability of the sensor along its body. \figref{fig:forcesensorstation_char} shows the force measurements at each phase of the experiment.
%\begin{figure}[t]
%  \begin{center}
%    \includegraphics[width=0.48\textwidth]{figures/forcesensorchar_battery.png}
%  \end{center}
%    \caption{The figure shows the force sensor readings when no object (blue line), one object (orange line) and two objects (green line) are applied to it. The results were converted from N to gram to ease the evaluation.}
%  \label{fig:forcesensorstation_char}
%\end{figure}
%The plotted graph shows accurate force measurements. Although there are some small variations due to noise in the measurement, the readings obtained from the sensor still follow the reference. Specifically, in the case of one object, the force sensor reported a mass of 107.65 g which is close to the ground truth mass of 108.2 g. For two objects, the real mass was 216.4 g and the sensor reported an average of 201.97 g. 
\subsection{Internal Force Characterization}
To characterize the internal force of the force sensor, a finger of \ourhand{} with integrated sensors was actuated in free space with a 60 kPa ramp input. Once the internal pressure in the finger reached 60 kPa, the input was zeroed, and the finger returned to its initial position. The top left plot in \figref{fig:forceestimator} shows the force measurement of the force sensor against the bending angle after 35 repetitions. Theoretically, the force measurements should remain zero as there is no contact between the finger and the environment. However, as seen in the figure, the force reading increases the more the finger is bent. Due to such sensor characteristics, the FSR force measurements of a bent finger are incorrect. Thus, removing the effect of the internal force from the sensor readings is crucial to enable force control of the fingers.  

\begin{figure*}
  \begin{center}
    \includegraphics[width=0.95\textwidth]{figures/internalforce.png}
  \end{center}
    \caption{The upper row (from left to right) shows, as blue dots, the internal force for each finger (from finger 1 to finger 3) at different bending angles along with the fitted polynomial model in red. The bottom row shows the BIC values for each finger.
}
  \label{fig:forceestimator}
\end{figure*}

\subsection{Contact Force Estimation}
\label{sec:calib_contact_force_est}
We model the actual contact force $F_{c}$ for the finger by the difference between the measured force $F_{m}$ and the internal force $F_{i}$
\begin{equation}
    F_{c} = F_{m} - F_{i}.
\label{contactforce_equation}
\end{equation}
Thus, to estimate the actual contact force $F_c$, we 1) learn the internal force $F_{i}$ caused by bending in free space and 2) subtract the estimated internal force from the measured force.

We cast the learning of the internal force model $F_{i}$ for each finger as a polynomial regression problem since the relationship between internal force and bending angle of the finger is non-linear (\figref{fig:forceestimator}). Thus the internal force is expressed as
\begin{equation}
     F_{i}(x) = \sum_{d=0}^{D} w_{d} x^{d}=\mathbf{w}^{\text{T}}\mathbf{x},
\label{eq:polymodel}
\end{equation}
where $\mathbf{w}=[w_1,\dots,w_D]$ are the parameters to learn, $x$ the bending angle of the finger, and $D$ the maximum degree of the polynomial function. We estimate the model parameters by first mapping the bending angle $x$ to a higher dimensional feature space using the feature map $\phi(x)= [x^{d},\dots,1]^{\text{T}}$, resulting in a transformed feature vector $\mathbf{x}=[x^{d},\dots,1]^{\text{T}}$, and then applying ordinary least squares so that the optimal parameters $\mathbf{w}^*$ can be found by $\mathbf{w}^{*} = (\mathbf{X}^T \mathbf{X})^{-1}\mathbf{X}^T \mathbf{F}_i$. 
% To simplify the  problem, the polynomial regression was interpreted as a combination of a feature map (transformation) and linear regression \cite{alexjung}.

To choose the model complexity, that is the maximum degree $D$ of the polynomial function, we used the \ac{bic} \cite{bic}
\begin{equation}
    \text{BIC} = \ln(n) k - 2 \ln(\hat{L}),
\end{equation}
where $\hat{L}$ is the maximized value of the likelihood of the model, $n$ is the number of observations, and $k$ is the number of parameters. The model with smallest BIC value is considered the best. 
%The reason the data for each finger are quite different from each other stems from the fabrication and sensor integration process, as this is done manually no finger is identical. Nevertheless, the $R^2$ values show that the predictive models fit the data very well. 

%Although \figref{fig:forceestimator} shows the predicted internal force against the real data and the error between the two.

%It is seen that the collected data from three fingers are different from each other. The main reason for this lies in the fabricating process of the finger, and the sensor integrating process as the processes are done manually and the fingers are not identical. This, in turn, leads to the variation in the collected data. Regardless of this matter, the $R^2$ values show that the predictive models fit the data very well. The predicted internal force will later be subtracted from the real force measurement from the sensor to estimate the actual contact force.  

% \jens{Maybe move the text below to a new subsection in the experiments called something like "Estimating contact force". Also, write in one sentence how you get the actual contact force}
% \begin{figure}[t]
%   \begin{center}
%     \includegraphics[width=0.48\textwidth]{figures/ext200.jpg}
%   \end{center}
%     \caption{Contact force estimation result of the force sensor.}
%   \label{fig:estimation_result}
% \end{figure}
% \figref{fig:estimation_result} plots the estimated contact force against the reference contact force for verifying the hypothesis. The plotted graph shows that the estimate contact force, \ie, slightly varies around the actual contact force. The error of this estimation, which ranges from 0.01 to 0.15 N at most, is within the tolerance for the objects we will later grasp. Therefore, the proposed assumption of estimating the contact force by simply subtracting the internal force from the real measurement is shown to be sufficiently accurate. This estimated contact force will later be used to detect the contact between the finger and objects. Due to the fluctuation of the estimation error, a certain threshold is set to safely detect contact between the finger and an external object. The value of the threshold is defined differently for different fingers according to their maximum value of the estimation error. 

